IRAS 00450+7401 and the mid-infrared fade/burst cycle of R Coronae Borealis-type stars

We present optical and infrared imaging and spectroscopy of the R Coronae Borealis-type (R Cor Bor) star IRAS 00450+7401. Optical spectra further confirm its classification as a cool R Cor Bor system, having a hydrogen-deficient carbon star spectral sub-class of HdC5 or later. Mid-infrared spectroscopy reveals the typical ~8 um ``hump'' seen in other R Cor Bor stars and no other features. A modern-epoch spectral energy distribution shows bright emission from hot dust having Tdust>600 K. Historical infrared data reveal generally cooler dust color temperatures combined with long-term fading trends, but provide no discernible correlation between flux level and temperature. Investigating the most mid-infrared variable R Cor Bor stars found in IRAS, AKARI, and WISE data reveals similar fading trends, bursts that can show a factor of up to 10 change in flux density between epochs, and blackbody-fit dust color temperatures that span 400-1300 K. While some R Cor Bor stars such as IRAS 00450+7401 appear to undergo fade/burst cycles in the mid-infrared, significant gaps in temporal coverage prevent conclusively identifying any preferred timescale for their mid-infrared variability and circumstellar dust temperature changes.

==> Acronyms.tex <==
% \acro{CEA}{Centre for Extragalactic Astronomy}
\acro{API}{Application Programming Interface}
\acro{APT}{Aperture Photometry Tool}
\acro{ARO}{Atmospheric Research Observatory}
\acro{ASU}{Arizona State University}
\acro{ASU}{Arizona Statue University}
\acro{AURA}{Association of Universities for Research in Astronomy}
\acro{AstOrb}{Asteroid Orbital Elements Database}
\acro{BLT}{Barry Lutz Telescope}
\acro{CADC}{Canadian Astronomy Data Centre}
\acro{CASU}{Cambridge Astronomy Survey Unit}
\acro{CATCH}{Comet Asteroid Telescopic Catalog Hub}
\acro{CBAT}{Central Bureau for Astronomical Telegrams}
\acro{CBET}{Central Bureau for Electronic Telegrams}
\acro{CCD}{charge-coupled device}
\acro{CEA}{Commissariat a l'Energes Atomique}
\acro{CFHT}{Canada France Hawaii Telescope}
\acro{CFHT}{Canada-France-Hawaii Telescope}
\acro{CNRS}{Centre National de la Recherche Scientifique}
\acro{COVID-19}{corona virus disease 2019} % 7/22/2022 COC
\acro{CSBN}{Committee for Small Bodies Nomenclature}
\acro{CTIO}{Cerro Tololo Inter-American Observatory}
\acro{DAPNIA}{Département d'Astrophysique, de physique des Particules, de physique Nucléaire et de l'Instrumentation Associée}
\acro{DART}{Double Asteroid Redirection Test}
\acro{DCT}{Discovery Channel Telescope}
\acro{DDT}{Director's Discretionary Time}
\acro{DECam}{Dark Energy Camera}
\acro{DESTINY+}{Demonstration and Experiment of Space Technology for INterplanetary voYage with Phaethon fLyby and dUst Science}
\acro{DES}{Dark Energy Survey}
\acro{DPRC}{Disability Program Resource Center}
\acro{DR}{Data Release}
\acro{DS9}{Deep Space Nine}
\acro{Dec}{Declination}
\acro{ELTE}{Eotvos Lorand University}
\acro{ESA}{European Space Agency}
\acro{ESO}{European Space Organization}
\acro{ETC}{exposure time calculator}
\acro{FAQ}{Frequently Asked Questions}
\acro{FITS}{Flexible Image Transport System}
\acro{FOV}{field of view}
\acro{GEODSS}{Ground-Based Electro-Optical Deep Space Surveillance}
\acro{GIF}{Graphic Interchange Format}
\acro{GMOS}{Gemini Multi-Object Spectrograph}
\acro{GRFP}{Graduate Research Fellowship Program}
\acro{HARVEST}{Hunting for Activity in Repositories with Vetting-Enhanced Search Techniques}
\acro{HPC}{High Performance Computing}
\acro{HSC}{Hyper Suprime-Cam}
\acro{IAS15}{Integrator with Adaptive Step-size control, 15th order}
\acro{IAU}{International Astronomical Union}
\acro{IMACS}{Inamori-Magellan Areal Camera and Spectrograph}
\acro{IMB}{inner Main-belt}
\acro{IMCCE}{Institut de Mécanique Céleste et de Calcul des Éphémérides}
\acro{INT}{Isaac Newton Telescopes}
\acro{IPAC}{Infrared Processing and Analysis Center}
\acro{IP}{Internet Protocol}
\acro{IRSA}{Infrared Science Archive}
\acro{ITC}{integration time calculator}
\acro{JAXA}{Japan Aerospace Exploration Agency}
\acro{JD}{Julian Date}
\acro{JFC}{Jupiter Family Comet}
\acro{JPL}{Jet Propulsion Laboratory}
\acro{KBO}{Kuiper Belt object}
\acro{KIDS}{Kilo-Degree Survey}
\acro{KOA}{Keck Observatory Archive}
\acro{KPNO}{Kitt Peak National Observatory}
\acro{LBCB}{Large Binocular Camera Blue}
\acro{LBCR}{Large Binocular Camera Red}
\acro{LBC}{Large Binocular Camera}
\acro{LBT}{Large Binocular Telescope}
\acro{LCO}{Los Cumbres Observatory}
\acro{LCOGT}{Las Cumbres Observatory Global Telescope}
\acro{LDT}{Lowell Discovery Telescope}
\acro{LINEAR}{Lincoln Near-Earth Asteroid Research}
\acro{LMI}{Large Monolithic Imager}
\acro{LONEOS}{Lowell Observatory Near-Earth-Object Search}
\acro{LSST}{Legacy Survey of Space and Time}
\acro{MBC}{Main-belt Comet}
\acro{MGIO}{Mount Graham International Observatory}
\acro{ML}{machine learning}
\acro{MMB}{middle Main-belt}
\acro{MOST}{Moving Object Search Tool}
\acro{MPC}{Minor Planet Center}
\acro{NASA}{National Aeronautics and Space Administration}
\acro{NAU}{Northern Arizona University}
\acro{NEAT}{Near-Earth Asteroid Tracking}
\acro{NEA}{near-Earth asteroid}
\acro{NEO}{near-Earth object}
\acro{NIHTS}{Near-Infrared High-Throughput Spectrograph}
\acro{NOAO}{National Optical Astronomy Observatory}
\acro{NOIRLab}{National Optical and Infrared Laboratory}
\acro{NONCOM}{Not Orbitally a Nominal Comet but Overtly a Minor planet}% 7/1/2022 COC
\acro{NRC}{National Research Council}
\acro{NSF}{National Science Foundation}
\acro{OMBA}{outer main-belt asteroid}
\acro{OMB}{outer Main-belt}
\acro{OSIRIS-REx}{Origins, Spectral Interpretation, Resource Identification, Security, Regolith Explorer}
\acro{PAC}{Physics and Astronomy Club}
\acro{PANSTARRS}{Panoramic Survey Telescope and Rapid Response System}
\acro{PI}{Principal Investigator}
\acro{PNG}{Portable Network Graphics}
\acro{PS1}{Panoramic Survey Telescope and Rapid Response System 1}
\acro{PSF}{point spread function}
\acro{PSI}{Planetary Science Institute}
\acro{PTF}{Palomar Transient Factory}
\acro{Pan-STARRS}{Panoramic Survey Telescope and Rapid Response System}
\acro{QHA}{Quasi-Hilda Asteroid}
\acro{QHC}{Quasi-Hilda Comet}
\acro{QHO}{Quasi-Hilda Object}
\acro{RA}{Right Ascension}
\acro{REU}{Research Experience for Undergraduates}
\acro{SAFARI}{Searching Asteroids For Activity Revealing Indicators}
\acro{SAO}{Smithsonian Astrophysical Observatory}
\acro{SBDB}{Small Body Database}
\acro{SDSS DR-9}{Sloan Digital Sky Survey Data Release Nine}
\acro{SDSS}{Sloan Digital Sky Survey}
\acro{SDSU}{San Diego State University}
\acro{SFSU}{San Francisco State University}
\acro{SLAC}{Stanford Linear Accelerator Center}
\acro{SMOKA}{Subaru Mitaka Okayama Kiso Archive}
\acro{SNR}{signal to noise ratio}
\acro{SOAR}{Southern Astrophysical Research Telescope}
\acro{SOFIA}{Stratospheric Observatory for Infrared Astronomy}
\acro{SQL}{Structured Query Language}
\acro{SSOIS}{Solar System Object Information Search}
\acro{STScI}{Space Telescope Science Institute}
\acro{SUP}{Suprime Cam}
\acro{SwRI}{Southwestern Research Institute}
\acro{TNO}{Trans-Neptunian object}
\acro{TRIF}{Technology and Research Initiative Fund} % an AZ thing
\acro{TSIP}{Telescope System Instrumentation Program}
\acro{TTU}{Texas Tech University}
\acro{UA}{University of Arizona}
\acro{UCB}{University of Colorado Boulder}
\acro{UCLA}{University of California Los Angeles}
\acro{UCSC}{University of California Santa Cruz}
\acro{UCSD}{University of California San Diego}
\acro{UCSF}{University of California San Francisco}
\acro{UT}{Universal Time}
\acro{VATT}{Vatican Advanced Technology Telescope}
\acro{VIRCam}{VISTA InfraRed Camera}
\acro{VISTA}{Visible and Infrared Survey Telescope for Astronomy}
\acro{VLT}{Very Large Telescope}
\acro{VST}{Very Large Telescope (VLT) Survey Telescope}
\acro{WCS}{World Coordinate System}
\acro{WFC}{Wide Field Camera}
\acro{WGSBN}{Working Group for Small Bodies Nomenclature}
\acro{WIRCam}{Wide-field Infrared Camera}
\acro{WISE}{Wide-field Infrared Survey Explorer}
\acro{YORP}{Yarkovsky--O'Keefe--Radzievskii--Paddack}
\acro{ZTF}{Zwicky Transient Facility}

